ROAD: The ROad event Awareness Dataset for Autonomous Driving

Humans drive in a holistic fashion which entails, in particular, understanding dynamic road events and their evolution. Injecting these capabilities in autonomous vehicles can thus take situational awareness and decision making closer to human-level performance. To this purpose, we introduce the ROad event Awareness Dataset (ROAD) for Autonomous Driving, to our knowledge the first of its kind. ROAD is designed to test an autonomous vehicle's ability to detect road events, defined as triplets composed by an active agent, the action(s) it performs and the corresponding scene locations. ROAD comprises videos originally from the Oxford RobotCar Dataset annotated with bounding boxes showing the location in the image plane of each road event. We benchmark various detection tasks, proposing as a baseline a new incremental algorithm for online road event awareness termed 3D-RetinaNet. We also report the performance on the ROAD tasks of Slowfast and YOLOv5 detectors, as well as that of the winners of the ICCV2021 ROAD challenge, which highlight the challenges faced by situation awareness in autonomous driving. ROAD is designed to allow scholars to investigate exciting tasks such as complex (road) activity detection, future event anticipation and continual learning. The dataset is available at https://github.com/gurkirt/road-dataset; the baseline can be found at https://github.com/gurkirt/3D-RetinaNet.

==> text/discussion.tex <==
% FAB: whether to fuse this with "Experiments" we can discuss
\section{DISCUSSION}
\label{sec:discussion}

[\emph{Do we want a separate discussion section, or we want discussion to follow each separate experiment in the related paragraph?}]

\subsection{Road user action vs human action}

\subsection{Joint vs marginal fusion inference}
 - We have these results now.
 
 - extension to weakly supervised learning

[any other suggestion]


==> text/soa_ad.tex <==
\section{RELATED WORK}
\label{sec:related_work} % \label{related_work:sec:st_det}

Initial attempts to perform space-time action detection were based on either action cuboid hypotheses and sliding-window based approaches~\cite{laptev2007retrieving,cao2010cross,tian2013spatiotemporal}, or
human location-centric based methods~\cite{prest2013explicit,lan2011discriminative,tian2013spatiotemporal,klaser2010human,wang2014video}.
These approaches were limited by the cuboidal shape of their action proposals or their reliance on human location information, respectively.
In opposition, unsupervised 3D action proposals-based methods~\cite{jain2014action,oneata2014spatio,Soomro2015,marian2015unsupervised} 
use a greedy agglomerative clustering of supervoxels for video segmentation, whose major drawback is that they are very expensive and impractical for long duration videos.

\iffalse
Initial attempts for space-time action detection were based on action cuboid hypotheses and sliding-window based approaches~\cite{laptev2007retrieving,cao2010cross,tian2013spatiotemporal}.
Major drawbacks of these methods are: 
(1) assumption that an action can be localised using a cuboidal video subvolume which is not realistic; 
(2) the video space is much larger ($\mathcal{O}(w^{2} h^{2} n^{2})$~\cite{tran2014video}) than the image space, and thus, a sliding-window scheme is extremely expensive. 
    
Human location-centric approaches~\cite{prest2013explicit,lan2011discriminative,tian2013spatiotemporal,klaser2010human,wang2014video} 
use human location information for action detection. 
On the other hand, unsupervised 3D action proposals based approaches~\cite{jain2014action,oneata2014spatio,Soomro2015,marian2015unsupervised} 
use a greedy agglomerative clustering of supervoxels for video segmentation for action detection.
The major drawback of unsupervised video segmentation methods is that they are very expensive and impractical for long duration videos,  or for applications requiring online and real-time processing.
For instance, it takes several minutes to segment a video clip of resolution $400 \times 720$ with a temporal length of $55$ frames~\cite{van2015apt}. 
%----------------------------------
The main issue with graph-based video segmentation is the irregular shape of supervoxels and their highly varying temporal extents~\cite{jain2014supervoxel}.   
Other issues with the above aproaches is that action region hypotheses 
with lower IoU overlap with ground truth tubes, leading to poor action localisation performance.  
%Supervoxels with highly varying temporal extents, instead, lead to brittle graphs.  

To alleviate the expensive video segmentation process, Van Gemert~\etal~\cite{van2015apt} and Yu~\etal~\cite{yu2015fast} completely bypass the video segmentation step.    
However, as the former generate action tubes by clustering motion features (i.e., dense trajectories~\cite{wang2011action}), it may not work on actions characterised by small motions.
Yu~\etal~\cite{yu2015fast}'s method, instead, a generic action proposal generation method which requires localised training samples, hence it is not scalable.
The main drawback for all the above method is that they reuire whole video at its disposal to detect action tubes, streaming or online processing is not feasible. % to online action tube detections. 
\fi
    
Frame-based action detection approaches~\cite{Georgia-2015a,Weinzaepfel-2015,Saha2016,peng2016eccv,singh2017online} demonstrated promising results.
These frameworks mainly leverage object detection algorithms~\cite{girshick-2014,ren2015faster} and the two-stream CNN framework~\cite{simonyan2014two} for action detection.
A frame-based feature representation, however, cannot encode the inter-frame temporal relationships between action regions spanning successive video frames. 
Thus, for linking the frame-level detections in time Viterbi (dynamic programming)~\cite{Georgia-2015a,Saha2016,peng2016eccv} or tracking algorithms~\cite{Weinzaepfel-2015} need to be used.
To put it differently, in frame-based methods the deep network is not in a condition to learn the temporal features essential for accurate action detection, and temporal reasoning is performed by some tube construction stage, in a suboptimal post-processing step. 
%However, Singh ~\etal show that online and real-time processing of videos possible
%Temporal features help encoding the complex motion pattern of human actions, i.e., allowing the network to understand how those actions evolve over time.

Recently, video-based action representation approaches have appeared~\cite{kalogeiton2017action,hou2017tube,hou2017end,saha2017amtnet} which
address this issue by learning complex non-linear functions (in the form of CNNs) which map video data (instead of image data) to a high dimensional latent feature space.
\\
Kalogeiton~\etal~\cite{kalogeiton2017action} and Hou~\etal~\cite{hou2017tube,hou2017end}'s models map $K$ video frames to such a latent space, 
whereas Saha~\etal~\cite{saha2017amtnet} only require $2$ successive frames to learn spatio-temporal feature embeddings.
The main advantage of~\cite{saha2017amtnet} over~\cite{kalogeiton2017action,hou2017tube} is that its framework is not constrained to process a fixed set of $K$ frames, but is
flexible enough to select training frame pairs $(f_{t}, f_{t+\Delta})$ at various intervals by varying the $\Delta$ value according to the requirements of a particular dataset
(i.e. a larger $\Delta$ for longer sequences, or a relatively smaller one for shorter video clips). 
This allows the system to leverage the sparse annotation provided with the latest generation action detection datasets, such as AVA~\cite{ava2017gu} and DALY~\cite{daly2016weinzaepfel}.
Another benefit of~\cite{saha2017amtnet}'s work is that it requires less computing time and resources both at train and test time.
\\
Our action detection framework does indeed adapt the network architecture of~\cite{saha2017amtnet} by advancing significant architectural changes, i.e.,
the use of a single-stage (SSD~\cite{liu15ssd}) faster base network, an added
motion stream, and a convolutional feature fusion layer
(discussed in detail in the next section).

So far we have discussed action detetion methods which mostly follow an offline setup, where it is assumed that the entire video clip is available to the system beforehand.
In most real world scenarios, however, this is not the case -- we thus need action detectors which can incrementally detect action instances from a partially observed video in an online fashion.
%A different direction of research focuses on online action detection.
Early online action prediction works have focussed on dynamic bags of words \cite{Earlyryoo2011human}, structured SVMs \cite{hoai2014max},
hierarchical representations \cite{lan2014hierarchical}, LSTMs and Fisher vectors \cite{de2016online}.
Unlike our framework, however, \cite{Earlyryoo2011human,hoai2014max,lan2014hierarchical} do not perform online action localisation. 
%FABIO: WE COULD STILL USE THEM AS BASELINE FOR THE PREDICTION BIT, RIGHT? 
Soomro~\etal~\cite{Soomrocvpr2016} have recently proposed an online method which can predict an action's label and location by observing a relatively smaller portion of the entire video sequence.
However, \cite{Soomrocvpr2016} only works on temporally trimmed videos and not in real-time, due to expensive segmentation.
Singh~\etal~\cite{singh2017online}, on the other hand, have brought forward an online action detection and early label prediction approach which works on temporally untrimmed videos.
Our online action tube generation algorithm is inspired by~\cite{singh2017online}'s approach. The main difference is that the method proposed here is designed to connect in time video-level action micro-tubes, rather than frame-level detection bounding boxes as in \cite{singh2017online}.

Finally, spatiotemporal 3D representation~\cite{carreira2017quo,tran2018closer,xie2018rethinking,nonlocal2018wang} has recently emerged as a dominant force in action detection~\cite{ava2017gu,girdhar2018video,duarte2018videocapsulenet}, amongst others.
Gu~\etal~\cite{ava2017gu}, for instance, combine an inflated 3D (I3D) network~\cite{carreira2017quo} with 2D proposals as in~\cite{peng2016eccv} 
to exploit the representational power of I3D. Similar concepts are proposed in~\cite{xie2018rethinking,girdhar2018video,li2018recurrent}. 
Duarte~\etal~\cite{duarte2018videocapsulenet}, instead, have proposed an interesting 3D video-capsule network for frame-level action segmentation which, however,
does not output action tubes and uses a different evaluation protocol.
\\
While our goal is to exploit 3D proposals to generate online action tubes, the above methods are inherently offline because of their use of temporal convolution.
Additionally, their contribution is mostly on the representation side, except~\cite{li2018recurrent},
whereas our main contribution is the notion of flexible 3D proposals. For these reasons, they are not directly comparable to our approach. 
We do provide a comparison with~\cite{li2018recurrent}, which uses 3D proposals generated by recurrent networks, showing better results on the UCF101 dataset. 


  
   

% ---------------------------------------------------------------------------------------------
% See related work section
\iffalse
\subsection{Action detection}
\label{sec:twotwo}

\noindent Recognising and localising, in space and time, different actions or events appearing in a streaming video is a crucial component of video understanding. In particular, autonomous vehicles needs to perceive the behaviour of other agents on road pedestrians on the side walk by identifying which kind of activities (e.g., ‘moving’ versus ‘waiting to cross’) they are performing, when and where this is happening. In the computer vision literature this problem is referred to as spatiotemporal action localisation or, in short, \emph{action detection}~\cite{georgia2015tube,ava2017gu,weinzaepfel2015learning,singh2017online,saha2017amtnet}.

\textcolor{r}{This section needs major rewrite. We need accommodate latest works on action detection and object detection in videos.}

There are many methods that perform action detection on frame-level~\cite{ava2017gu} on AVA~\cite{ava2017gu} or UCF24~\cite{soomro2012ucf101,singh2017online}.

State of the art methods in this field work by constructing \textit{action tubes}, {i.e.}, sequences of detection bounding boxes around the action of interest, linked in time. In particular, regions potentially containing the instance of a relevant action are fed to specific classifiers, which make predictions using both static (appearance) and dynamic (motion, typically represented by optical flow) cues. Then, these regions are linked across frames based on the predicted action labels and their spatial overlap, in order to produce action tubes for each action instance within the video. Action detection is generally performed using a multi--region two--stream recursive convolutional neural network (R-CNN) model. Building on the frame--level action detection method based on Faster R-CNN \cite{ren2015faster}, many authors have proposed to exploit the high-quality results generated by a motion region proposal network, which are complementary to those of an appearance region proposal network. Stacking optical flow images over several frames, in particular, shows significant improvements over frame-level action detection.  

Although a considerable amount of research has been undertaken in this area, the majority of approaches perform action tube generation in an \emph{offline} fashion, and are thus not suitable for application to real world scenarios such as self--driving cars, which require the online processing of streaming video frames at real-time speed. 

\noindent More recent efforts try to address the problem of action detection by predicting \textit{micro-tubes}~\cite{saha2017amtnet}. In this way, the network itself learns the temporal connection between bounding boxes belonging to pairs of successive video frames at a certain temporal distance. However, micro-tubes need to be linked together, and this is still done in an offline fashion, after that the entire video is available. 
% Gurkirt: It is wrong removing it
 \noindent Another interesting approach is that proposed by Kalogeiton \textit{et al.}~\cite{kalogeiton2017action}. Their Action Tubelet detector takes as input a sequence of frames and produces as output \textit{tubelets}, {i.e.}, sequences of bounding boxes with attached a confidence score per action class. This approach too, however, assumes video frames are available beforehand.
\fi 

